Explaining Deep Neural Networks

Deep neural networks are becoming more and more popular due to their revolutionary success in diverse areas, such as computer vision, natural language processing, and speech recognition. However, the decision-making processes of these models are generally not interpretable to users. In various domains, such as healthcare, finance, or law, it is critical to know the reasons behind a decision made by an artificial intelligence system. Therefore, several directions for explaining neural models have recently been explored. In this thesis, I investigate two major directions for explaining deep neural networks. The first direction consists of feature-based post-hoc explanatory methods, that is, methods that aim to explain an already trained and fixed model (post-hoc), and that provide explanations in terms of input features, such as tokens for text and superpixels for images (feature-based). The second direction consists of self-explanatory neural models that generate natural language explanations, that is, models that have a built-in module that generates explanations for the predictions of the model.

==> abbrev.tex <==
\begin{abbrev}


MLP .............. Multilayer Perceptron \\
SGD .............. Stochastic Gradient Descent \\
SNLI ............. Stanford Natural Language Inference \\
ReLU ............  Rectified Linear Unit \\
CNN .............. Convolutional Neural Network \\
RCNN ............  Recurrent Neural Network  \\
LSTM ............. Long Short Term Memory \\
GRU .............. Gated Recurrent Unit \\

\end{abbrev}

==> journey.tex <==
\begin{journey}
This thesis summarizes my main topic of research as a DPhil student in the Department of Computer Science at the University of Oxford, under the supervision of Prof. Phil Blunsom and Prof. Thomas Lukasiewcz. While, in this manuscript, I will only present my research on explaining deep neural networks, my DPhil journey was much more diverse, hence I would like to briefly mention the other projects and people that have made me grown as a researcher. 

In my first year of DPhil, I had the exciting opportunity to undertake a research internship in the Machine Perception team at Google, Mountain View, under the supervision of Dr. Alexander Toshev. There, I have worked on a project of generation and comprehension of unambiguous object descriptions in natural images \citep{DBLP:journals/corr/MaoHTCYM15}. This wonderful experience has given me first hand experience with research in industry.

Throughout the following years, I also had the amazing opportunity to co-supervise three MSc students on diverse projects:
\begin{itemize}
    \item Learning Disentangled Word Embeddings (Ana-Maria Cretu, visiting MSc student from the École Polytechnique Fédérale de Lausanne, Sept. 2017 - Aug. 2018)
    \item Natural Language Hypothesis Generation with Natural Language Explanations (Vlad Barvinko, MSc student at the University of Oxford, May - Aug. 2019)
    \item Visual Entailment with Natural Language Explanations (Virginie Do, MSc student at the University of Oxford, May - July 2019). 
\end{itemize}

Further, in the last year of my DPhil, I have also co-supervised Vid Kocijan, at the time in his first year of DPhil in our group. We worked on the topic of co-reference resolution \citep{vid-emnlp} and commonsense reasoning \citep{vid-acl}. We are currently still collaborating on a project of gender bias in co-reference resolution which we submitted at ACL 2020.

The experience of co-supervising younger researchers has been extremely rewarding and has helped me grow not only as a researcher but also as a mentor. 

In addition, I also had the delightful opportunity to be a reviewer for NeurIPS 2019, which improved my constructive critical skills.

Finally, the roles I held both in the department (Secretary and Outreach Office in the Oxford Women in Computer Science society), and in my college (Art Representative, President of the Linacre College Tennis Society, and Head Resident), have polished my management and leadership skills.

Hence, the DPhil journey was diverse, life-forming, and rewarding, and I would like to express my gratitude to all the people that have contributed to make it possible. % and a fruitful experience.


\end{journey}
